Diffusion Model-Augmented Behavioral Cloning

Imitation learning addresses the challenge of learning by observing an expert's demonstrations without access to reward signals from environments. Most existing imitation learning methods that do not require interacting with environments either model the expert distribution as the conditional probability p(a|s) (e.g., behavioral cloning, BC) or the joint probability p(s, a). Despite the simplicity of modeling the conditional probability with BC, it usually struggles with generalization. While modeling the joint probability can improve generalization performance, the inference procedure is often time-consuming, and the model can suffer from manifold overfitting. This work proposes an imitation learning framework that benefits from modeling both the conditional and joint probability of the expert distribution. Our proposed Diffusion Model-Augmented Behavioral Cloning (DBC) employs a diffusion model trained to model expert behaviors and learns a policy to optimize both the BC loss (conditional) and our proposed diffusion model loss (joint). DBC outperforms baselines in various continuous control tasks in navigation, robot arm manipulation, dexterous manipulation, and locomotion. We design additional experiments to verify the limitations of modeling either the conditional probability or the joint probability of the expert distribution, as well as compare different generative models. Ablation studies justify the effectiveness of our design choices.

==> figure/ablation_study.tex <==
\begin{figure*}[t]
    % \vspace{-10pt}
    \centering
    \begin{subfigure}[b]{0.20\textwidth}
    \label{fig:coefficient}
    \centering
    \includegraphics[width=\textwidth, height=\textwidth]{figure/ablation_study/coefficient.jpeg}
    % \caption{\textsc{coefficient}}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.20\textwidth}
    \label{fig:agent_only}
    \centering
    \includegraphics[width=\textwidth, height=\textwidth]{figure/ablation_study/agent_only.png}
    % \caption{\textsc{agent_only}}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.20\textwidth}
    \label{fig:action_only}
    \centering
    \includegraphics[width=\textwidth, height=\textwidth]{figure/ablation_study/action_only.png}
    % \caption{\textsc{action_only}}
    \end{subfigure}
    % \hfill
    % \vspace{-5pt}
    \caption{\textbf{Ablation Study}:
    \textbf{(a) \textsc{coefficient}}:
    \textbf{(b) \textsc{agent_only}}: 
    \textsc{(c) \textsc{action_only}}:
    }
    \label{fig:ablation}
    % \vspace{-5pt}
\end{figure*}

==> figure/coefficient_ablation.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=0.7\textwidth]{figure/maze_coeff.png}    
    \includegraphics[width=0.3\textwidth]{figure/maze_coeff.png}
    \caption{\textbf{Effect of $\lambda$.} 
We experiment with different values of $\lambda$ in \maze{},
each evaluated over three random seeds.
% Setting $\lambda_{\text{BC}}=1$ and $\lambda_{\text{DM}}=1$ achieves the best performance.
}
    \label{fig:maze_coeff}
\end{figure}


==> figure/demos.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figure/demos_pdf.pdf}
\caption[Qualitative Results]{
    \textbf{Qualitative Results.}  
    Rendered videos of the policies learned by our proposed framework and the baselines can be found at    \url{https://nturobotlearninglab.github.io/dbc/}.
    \label{fig:demos}
}
\end{figure*}

==> figure/distance_succ.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.30\textwidth]{figure/distance_succ/bc.jpeg}
    \includegraphics[width=0.30\textwidth]{figure/distance_succ/vae_bc.jpeg}
    \includegraphics[width=0.30\textwidth]{figure/distance_succ/diff_bc.jpeg}
    \caption[\textbf{\maze{} Goal Distance Analysis}]{\textbf{\maze{} Goal Distance Analysis.} We compare the success rates of the baselines and our proposed method regarding the distance between the start point and the goal. The success rates of BC and VAE-BC decrease significantly as the distance range increases, while the success rate of our method \method{} remains relatively consistent.}
    \label{fig:distance_succ}
\end{figure*}

==> figure/len_curve.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.65\textwidth]{figure/result/legend_len.jpeg} 
    \vspace{0.2cm}
    \\
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]
    {figure/result/MazeLen.png}
    \caption{\textbf{\maze{}}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]
    {figure/result/FetchPickLen.png}
    \caption{\textbf{\fetchpick{}}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]
    {figure/result/HandLen.png}
    \caption{\textbf{\handrotate{}}}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]
    {figure/result/AntLen.png}
    \caption{\textbf{\antreach{}}}
    \end{subfigure}
    % \\ 
    % {\includegraphics[width=0.65\textwidth]{figure/result/legend_bc_diff_vae.pdf}}
    \caption[\textbf{Episode Length of Goal-Directed Tasks}]{\textbf{Episode Length of Goal-Directed Tasks.} We evaluate the baselines and our proposed method regarding the episode length during the learning process. Since Implicit BC ({\color[RGB]{84, 158, 63}green}) and Diffusion Policy ({\color[RGB]{165, 94, 52}brown}) take significantly longer to converge, we set a higher number of training epochs for these two methods, and hence their learning curves are notably longer than BC ({\color[RGB]{239, 134, 50}orange}) and \method{} (\textcolor{myblue}{blue}). The average episode length indicates how fast the agent reaches the goal, which can be a measurement of the efficiency of the agent.
    Our method \method{} demonstrates superior efficiency in accomplishing tasks.
    % Therefore, our method (\method{} in \textcolor{myblue}{blue}) demonstrates superior learning efficiency and is more robust to overfitting.
    }
    \label{fig:len_curve}
\end{figure*}

==> figure/training_curve.tex <==
\definecolor{myblue}{RGB}{18, 110, 168}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\textwidth]{figure/result/legend_len.jpeg} 
    \vspace{0.2cm}
    \\
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
    \includegraphics[width=\textwidth]
    {figure/result/Maze.png}
    \caption{\textbf{\maze{}}}
    \label{fig:maze_training}
    \end{subfigure}
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
    \includegraphics[width=\textwidth]
    {figure/result/FetchPick.png}
    \caption{\textbf{\fetchpick{}}}
    \label{fig:pick_training}
    \end{subfigure}
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
    \includegraphics[width=\textwidth]
    {figure/result/Hand.png}
    \caption{\textbf{\handrotate{}}}
    \label{fig:hand_training}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
    \includegraphics[width=\textwidth]
    {figure/result/Cheetah.png}
    \caption{\textbf{\cheetah{}}}
    \label{fig:cheetah_training}
    \end{subfigure}
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
    \includegraphics[width=\textwidth]
    {figure/result/Walker.png}
    \caption{\textbf{\walker{}}}
    \label{fig:walker_training}
    \end{subfigure}
    \begin{subfigure}[t]{0.28\textwidth}
    \centering
    \includegraphics[width=\textwidth]
    {figure/result/Ant.png}
    \caption{\textbf{\antreach{}}}
    \label{fig:ant_training}
    \end{subfigure}
    
    % \\
    % \adjustbox{trim={.0\width} {.13\height} {.0\width} {.13\height},clip}%
    % {\includegraphics[width=0.65\textwidth]{figure/result/legend.pdf}}
    % \vspace{-0.3cm}
    \caption[\textbf{Learning Progress.}]{\textbf{Learning Progress.}
    We evaluate the baselines and our proposed method \method{} and its variants during the learning process. Since Implicit BC ({\color[RGB]{84, 158, 63}green}) and Diffusion Policy ({\color[RGB]{165, 94, 52}brown}) take significantly longer to converge, we set a higher number of training epochs for these two methods, and hence their learning curves are notably longer than BC ({\color[RGB]{239, 134, 50}orange}) and \method{} (\textcolor{myblue}{blue}). Our method demonstrates superior learning efficiency over the baselines.
    }
    \label{fig:curve}
\end{figure}

==> figure/traj.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
    \centering
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/diff_2_0.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/bc_2_100.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/bc_2_200.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/bc_2_300.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/bc_2_365.png}
    \caption{BC} 
    \end{subfigure}
    \\
    \vspace{0.5cm}
    \begin{subfigure}[b]{1.0\textwidth}
    \centering
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/diff_2_0.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/ae_2_100.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/ae_2_200.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/ae_2_235.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/ae_2_235.png}
    \caption{VAE-BC} 
    \end{subfigure}
    \\
    \vspace{0.5cm}
    \begin{subfigure}[b]{1.0\textwidth}
    \centering    \includegraphics[width=0.18\textwidth]{figure/traj_vis/diff_2_0.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/diff_2_100.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/diff_2_181.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/diff_2_181.png}
    \includegraphics[width=0.18\textwidth]{figure/traj_vis/diff_2_181.png}
    \caption{\method{}} 
    \end{subfigure}
    % \\
    % \adjustbox{trim={.0\width} {.13\height} {.0\width} {.13\height},clip}%
    % {\includegraphics[width=0.65\textwidth]{figure/result/legend.pdf}}
    \caption[\textbf{\maze{} Trajectories}]{\textbf{\maze{} Trajectories.} \textbf{BC}: the agent takes 365 steps to reach the goal. \textcolor{red}{\textbf{VAE-BC}}: the agent takes 252 steps to reach the goal. \textbf{\method{}}: the agent takes 181 steps to reach the goal. The above results justify the effectiveness of our proposed method against the baselines. 
    }
    \label{fig:traj}
\end{figure*}

==> table/expert_norm_ablation.tex <==
\begin{table*}
\centering
\caption[\textbf{Effect of the Normalization Term}]{\textbf{Effect of the Normalization Term.} We aim to investigate whether normalizing the diffusion model loss $\mathcal{L}_{\text{DM}}$ with the expert diffusion model loss $\mathcal{L}_{\text{diff}}^{\text{expert}}$ yields improved performance.
We train a variant of \method{} where only $\mathcal{L}_{\text{diff}}^{\text{agent}}$ in~\myeq{eq:agent_loss} instead of $\mathcal{L}_{\text{DM}}$ in~\myeq{eq:dm_loss} is used to augment BC. We report the mean and the standard deviation of success rate (\maze{}, \fetchpick{}, \handrotate{}, \antreach{}) and return (\cheetah{}, \walker{}), evaluated over three random seeds.
}
\scalebox{0.9}{\begin{tabular}{@{}ccccc@{}}\toprule
\textbf{Environment} & $\mathcal{L}_{\text{diff}}^{\text{agent}}$ &  $\mathcal{L}_{\text{DM}}$\\
\cmidrule{1-3}
\maze{} & 94.7\% $\pm$ 1.9\%
& 95.4\% $\pm$ 1.7\%\\
\fetchpick{} & 96.6\% $\pm$ 1.7\%
& 96.9\% $\pm$ 1.7\%\\
\handrotate{} & 59.4\% $\pm$ 2.1\%
& 60.1\% $\pm$ 4.4\%\\
\antreach{} & 70.1\% $\pm$ 4.9\%
& 70.0\% $\pm$ 5.0\%\\
\cheetah{} & 4821.4 $\pm$ 124.0
& 4909.5 $\pm$ 73.0\\
\walker{} & 6976.4 $\pm$ 76.1
& 7034.6 $\pm$ 33.7\\
\bottomrule
\end{tabular}}
\label{table:expert_normalization1}
\end{table*}

==> table/len.tex <==
\begin{table*}
\centering
\caption[\textbf{Episode Length of Goal-Directed Tasks}]{\textbf{Episode Length of Goal-Directed Tasks.}
\hcw{We report the mean and the standard deviation of 
the episode length ($\downarrow$)
on \maze{}, \fetchpick{}, \handrotate{}, and \antreach{},
evaluated over three random seeds.
The experiments demonstrate that our proposed method (\method{}) performs competitively against the best-performing baselines (BC and Diffusion Policy) in all goal-directed tasks (\maze{}, \fetchpick{}, \handrotate{}, and \antreach{}).\hmh{Can make this part simpler}}
}
\scalebox{0.9}{\begin{tabular}{@{}ccccc@{}}\toprule
\textbf{Method} & 
\maze{} &
\fetchpick{} &
\handrotate{} &
\antreach{} \\ 
\cmidrule{1-5}
BC & 184.6 $\pm$ 9.9 
& 34.4 $\pm$ 1.0
& \textbf{33.1} $\pm$ 1.0 
& \textbf{39.0} $\pm$ 0.8 \\ 
Implicit BC & 205.8 $\pm$ 15.7 
& 44.7 $\pm$ 0.5
& 46.1 $\pm$ 1.2
& 45.5 $\pm$ 1.0 \\ 
Diffusion Policy & \textbf{172.0} $\pm$ 6.3
& 37.3 $\pm$ 0.5
& \textbf{31.4} $\pm$ 1.1
& 41.3 $\pm$ 0.8 \\ 
\method{} (Ours) & \textbf{176.2} $\pm$ 8.2
& \textbf{33.7} $\pm$ 0.4
& \textbf{32.1} $\pm$ 1.5
& \textbf{38.9} $\pm$ 0.8 \\ 
\bottomrule
\end{tabular}}
\label{table:len}
\end{table*}


==> table/maze_generalization.tex <==
\begin{table*}
\centering
\caption[]{\textbf{\maze{} Maze Generalization Experimental Result.}
We report the mean and the standard deviation of success rate of different goal coverage of \maze{}.
}
\scalebox{0.78}{\begin{tabular}{@{}ccccc@{}}\toprule
\textbf{Dataset Size} & 
100 &
75 &
50 &
25 \\
\cmidrule{1-5}
BC & 92.1\% $\pm$ 3.6\% 
& 89.7\% $\pm$ 2.5\% 
& 67.9\% $\pm$ 5.8\% 
& 50.7\% $\pm$ 5.5\% \\
Implicit BC & 78.3\% $\pm$ 6.0\% 
& 72.2\% $\pm$ 4.5\% 
& 65.2\% $\pm$ 3.2\% 
& 40.5\% $\pm$ 4.9\%  \\
Diffusion Policy & \textbf{95.5}\% $\pm$ 1.9\% 
& \textbf{89.5}\% $\pm$ 2.9\% 
& \textbf{71.2}\% $\pm$ 6.3\% 
& 52.3\% $\pm$ 5.4\% \\
\method{}  (Ours) & \textbf{95.4}\% $\pm$ 1.7\% 
& \textbf{89.2}\% $\pm$ 3.1\% 
& \textbf{69.8}\% $\pm$ 2.9\% 
& \textbf{57.7}\% $\pm$ 4.7\% \\
\bottomrule
\end{tabular}}
\label{table:maze_generalization}
\end{table*}

==> text/7_ack.tex <==
\section*{Acknowledgement}
\label{sec:ack}

This work was supported by the National Science and Technology Council, Taiwan (NSTC 112-2222-E-002-006-).
Shao-Hua Sun was supported by the Yushan Fellow Program by the Ministry of Education, Taiwan. 
